Learning about a changing state

A long-lived Bayesian agent observes costly signals of a time-varying state. He chooses the signals' precisions sequentially, balancing their costs and marginal informativeness. I compare the optimal myopic and forward-looking precisions when the state follows a Brownian motion. I also compare the myopic precisions induced by other Gaussian processes.

==> proofs/posterior.tex <==
\begin{proof}
    Consider the vector~$z=(y_n,\theta(t))\in\R^{n+1}$ obtained by appending~$\theta(t)$ to~$y_n$.
    This vector is multivariate normally distributed with mean~$\E[z]=(\E[y_n],\E[\theta(t)])$ and covariance matrix
    \[ \Var(z)=\begin{bmatrix}
        \Var(\theta(t)) & w_{nt}^T \\
        w_{nt}^T & \Sigma_n
    \end{bmatrix}. \]
    The result follows immediately from Lemma~\ref{lem:multivariate-normal-conditional}.
\end{proof}

